Compositional Task-Oriented Parsing as Abstractive Question Answering

Task-oriented parsing (TOP) aims to convert natural language into machine-readable representations of specific tasks, such as setting an alarm. A popular approach to TOP is to apply seq2seq models to generate linearized parse trees. A more recent line of work argues that pretrained seq2seq models are better at generating outputs that are themselves natural language, so they replace linearized parse trees with canonical natural-language paraphrases that can then be easily translated into parse trees, resulting in so-called naturalized parsers. In this work we continue to explore naturalized semantic parsing by presenting a general reduction of TOP to abstractive question answering that overcomes some limitations of canonical paraphrasing. Experimental results show that our QA-based technique outperforms state-of-the-art methods in full-data settings while achieving dramatic improvements in few-shot settings.

==> background.tex <==
\section{Background}
\subsection{Seq2seq Models and Denoising Objectives}
A seq2seq model defines an (estimated) probability distribution over a sequence of tokens $\bm{y} = y_1, \hdots, y_n$ conditioned on $\bm{x}$.
By the chain rule of probability, we can factorize this distribution as: 
\begin{align*}
p(\bm{y}|\bm{x}) &= \prod_{i=1}^n p(y_i \mid \bm{x}, y_1, \hdots, y_{i-1}). \label{eq:lm}
\end{align*}

State-of-the-art seq2seq models such as T5~\cite{raffel2020exploring} and BART~\cite{lewis2020bart} are pretrained on massive online corpora, through which they gain much language knowledge that can be leveraged in downstream tasks.
Their training objectives are to maximize their likelihood on training data and to denoise.
One common way of denoising is to randomly replace some parts of a text with mask tokens and have the models to recover the exact words.
We note that unlike some LMs such as BERT~\cite{devlin-etal-2019-bert} where their mask tokens only mask out one token, the denoising mask tokens can correspond to an arbitrary number of tokens.

We can fine-tune thee seq2seq models to perform semantic parsing.
The most straightforward way is to have them directly generate the structured meaning representation of an utterance; however, this involves generating entity symbols that are not seen by the models during pretraining.
%Although the end goal of semantic parsing is to generate a logical form that can be understood by machines, we can explore how the seq2seq models work with different natural language representations of the logical form
Therefore, generating a natural language representation of a semantic parse is more friendly to the models.
Since these models behave like black boxes and thus it is hard to know how it performs at generating different sequences, it becomes an interesting question how to best formulate the natural language representation of a semantic parse.

\subsection{Abstractive Question-answering}
A question-answering task is often to produce an answer to a question that is raised from a context.
Abstractive QA is one challenging form of QA tasks, where its answer is generated in free-form natural language in that it doesn't necessarily relying on the vocabulary of the question or document content, as opposed to extractive QA, where the answer is simply a span of the context.
Well-known examples of abstractive QA datasets include NarrativeQA~\cite{kovcisky2018narrativeqa}, QnA~\cite{nguyen2016ms}, and TWEETQA~\cite{xiong2019tweetqa}.

%Abstractive QA can be naturally formulated as a seq2seq task, where the input is the context and the question, and the output is the answer.
Abstractive QA is the most expressive form of QA tasks, as all other forms of QA tasks can be reduced to abstractive QA~\cite{khashabi2020unifiedqa}.
The reduction is done by treating abstractive QA as a seq2seq task, where the input is the context and the question, and the output is the answer, so that any QA task can be represented in this template.
We thus reformulate TOSP as abstractive QA, since it is able to deal with most complex structures. 
